Intersymbol and Intercarrier Interference in OFDM Systems: Unified Formulation and Analysis

A new unified formulation for seven different orthogonal frequency-division multiplexing (OFDM) systems is presented. The proposed formulation relies on six parameters and encompasses conventional OFDM systems, with windowing in the transmitter and/or in the receiver, and also with a cyclic prefix (CP) or both a CP and cyclic suffix (CS). A new equivalent channel matrix that is useful for calculating both the received signal and the intersymbol and intercarrier interference power is defined and characterized. Unlike previous works, this new channel matrix formulates the channel convolution with no restrictions on the length of the channel impulse response. Moreover, it includes the overlap-and-add procedure performed in the transmitter of windowed OFDM systems. Furthermore, new theoretical expressions for the intersymbol and intercarrier interference and also for the signal-to-interference-plus-noise ratio are derived.

==> Experimental_study_vehA_jun_2023.tex <==

\input{table_par_sim}

\section{Simulations}\label{sec:experiments}
In order to demonstrate the applicability of the proposed \fcro{unified} formulation, this section compares the performance of the studied systems in terms of SER and achievable data rate. It is worth noting that OOB emissions will not be taken into account here. The set of parameters used in the simulations are summarized in Table \ref{parameter_simulat}. BPSK modulation is used as the primary mapping, the number of active subcarriers is $N = 256$, which is the DFT size, and the frequency spacing is $11.16071492$ kHz. \fcr{One set of 250 wireless fading channels, according to the ITU Vehicular A channel \cite{Itu97, 3GPP07}, is used} as multipath channels. They have been generated with Matlab's \texttt{stdchan} using \fcr{the channel model \texttt{itur3GVAx} with a carrier frequency $f_{\rm c}=2$ GHz and \fcr{the following set of parameters:} 100 km per hour as mobile speed, $T_{\rm s}=200$~ns and  length $L=\nu+1=21$. These channels are referred to as VEH200}. The noise is \wam{modeled} as an additive white Gaussian noise. It is assumed that the channel remains unchanged within the same simulation and perfect channel estimation is performed at the receiver. Perfect time and frequency synchronization is also assumed. 


\begin{figure}%[!htb]
\centering{
{\includegraphics[width=0.45\textwidth]{figs/Fig-SER-Todos-VEH200.eps} \hfill \label{fig-SER_longi_VehA200}}
} 
\caption{SER versus SNR for different OFDM systems.}
\label{fig_SER_snr_values}
\end{figure}

In Fig. \ref{fig_SER_snr_values}, the ${\rm SER}$ performance curves of the different OFDM systems and channels are depicted. As can be seen, the results are practically indistinguishable for \fcr{this} set of channels. Thus, there is no clear advantage in terms of SER of any particular OFDM system over the other systems.  

\begin{figure}%[!htb]
\centering{
{\includegraphics[width=0.42\textwidth]{figs/Fig-Data-Rate-todos-VEH200.eps}  \label{fig-Data_rate_VehA200}}
} 
\caption{Total achievable data rate versus SNR for different OFDM systems.}
\label{fig_Data_rate_snr_values}
\end{figure}

%\input{table2}

\begin{figure}%[!htb]
\centering{
{\includegraphics[width=0.45\textwidth]{figs/Fig-SER-vs-Length-CP-Todos-SNR-VehA200-promedio.eps}  \label{fig-SER_longi_CP_VehA200}}
} 
\caption{SER versus CP length for different OFDM systems.}
\label{fig_SER_longi_CP_values}
\end{figure}


Next, we investigate the data rate performance for a fixed CP length ($\mu=32$). As we use BPSK modulation, the data rate for subcarrier $k$  is given by \cite{Gar06}
\begin{equation}\label{eq_capacityDCT}
C \left( k \right)= \frac{1}{2} \log _2 \left( {\frac{{{\rm SINR}\left( k \right)}}{\gamma ^ {\ast} }} \right),
\end{equation}
where $\gamma ^ {\ast}$ is the modified ${\rm SINR}$ gap defined for a target SER as
\[
\gamma ^{\ast} = \left( {\frac{{Q^{ - 1} \left( {{{\rm SER} \mathord{\left/
 {\vphantom {{\rm SER} 2}} \right.
 \kern-\nulldelimiterspace} 2}} \right)}}{{\sqrt 2 \pi }}} \right)^2 .
\]

\begin{figure}
\centering
\subfigure[]{\includegraphics[width=0.42\textwidth]{figs/Fig-Data-Rate-Todos-SNR-5-VehA200-promedio.eps}  \label{fig-longi_vehA200_SNR_5}}\hfill
\subfigure[]{\includegraphics[width=0.42\textwidth]{figs/Fig-Data-Rate-Todos-SNR-25-VehA200-promedio.eps}  \label{fig-longi_vehA200_SNR_25}}\hfill
\subfigure[]{\includegraphics[width=0.42\textwidth]{figs/Fig-Data-Rate-Todos-SNR-40-VehA200-promedio.eps}  \label{fig-longi_vehA200_SNR_45}}
\caption{Achievable data rate for different lengths for the CP and SNR values. }
\label{fig-data_rate_longi_snr_values}
\end{figure}


\begin{figure}
\centering
\subfigure[]{\includegraphics[width=0.45\textwidth]{figs/Fig-PICI1-todos-VEH200-SNR=varios.eps}  \label{fig-PICI1_longi_vehA200_SNR_5}}\hfill
\subfigure[]{\includegraphics[width=0.45\textwidth]{figs/Fig-PICI2-todos-VEH200-SNR=varios.eps}  \label{fig-PICI1_longi_vehA200_SNR_25}}\hfill
\subfigure[]{\includegraphics[width=0.45\textwidth]{figs/Fig-PISI-todos-VEH200-SNR=varios.eps}  \label{fig-PICI1_longi_vehA200_SNR_45}}
\caption{Total power for different CP lengths. (a) Power of type-I intercarrier interference. (b) Power of type-II intercarrier interference. (c) Power of intersymbol interference.}
\label{fig-Pvarios_longi_snr_values}
\end{figure}


The total achievable data rate is thus
\begin{equation}\label{eq_throughputDCT}
R = f_{\rm s} \sum\limits_{k = 0}^{N - 1} {\frac{N}{{N_0}} \cdot C\left( k \right)} ,
\end{equation}
where $N_0=N+\mu+\rho$ and $f_{\rm s}={1 \mathord{\left/
 {\vphantom {1 {T_{\rm s}}}} \right.
 \kern-\nulldelimiterspace} {T_{\rm s}}}$. We employ the SER obtained in the previous simulations to compute the values of $\gamma ^{\ast}$ corresponding to each SNR. Fig. \ref{fig_Data_rate_snr_values} shows the resulting data rate as a function of the SNR. In this set of experiments, the OFDM systems that offer the best results are CP, wrx and CPwrx. The systems performing windowing in the receiver and 
including a prefix and suffix, such as WOLA and CPW, offer a
lower \fcro{data} rate due to the penalty of adding the two
types of redundant samples.%Those systems that also have a window in the receiver, but include a prefix and suffix, such as WOLA and CPW, offer a lower transmission rate due to the penalty of including both types of redundant samples.  
 


We now analyze the influence of the CP size on the resulting data rate. To this purpose, the SER as a function of the CP length is obtained for each OFDM system (see Fig. \ref{fig_SER_longi_CP_values}), assuming ${\rm SNR} = 5, 25$, and $40$~dB. These results are employed to calculate $\gamma^{\ast}$. Then, we obtain the achievable data rate, depicted in Fig. \ref{fig-data_rate_longi_snr_values}.  In all cases, CP-OFDM outperforms the other systems, except for ${\rm SNR} = 40$~dB, and for smaller values of the CP, for which the wrx scheme shows a better performance. However, this improvement is not very significant in this case of insufficient redundant samples. The remaining OFDM systems have better performance whenever the windowing is in the \fcro{Rx}. For both small CP lengths and low SNR values, the systems that only have a CP outperform those that incorporate a CS.%For the rest of the schemes, a better performance can be seen in those that have a window in the receiver, as opposed to its counterpart that includes a window in the transmitter. For both low lengths of CP and low SNR values, the systems that only have CP outperforms those that also incorporate CS.


Finally, the formulation presented here allows analysis in the transform domain of the three different interference powers that appear in each OFDM scheme. %Figs. \ref{fig-PICI1_longi_snr_values}, \ref{fig-PICI2_longi_snr_values}, and \ref{fig-PISI_longi_snr_values} show the total power results ($P_{\rm ICI1}$, $P_{\rm ICI2}$, and $P_{\rm ISI}$) as a function of the CP length, obtained in the previous experiment for the case of ${\rm SNR} =$ \WAM{5, 25, 40~dB,} and the VEH200 channel. 
Fig. \ref{fig-Pvarios_longi_snr_values} shows the total power results ($P_{\rm ICI1}$, $P_{\rm ICI2}$, and $P_{\rm ISI}$) as a function of the CP length. The interference power is higher for systems whose windowing is performed in the \fcro{Tx} than those with windowing in the \fcro{Rx}. Note that \fcro{CPW-OFDM} has low levels of interference power, but the data rate results do not outperform the other systems. This is due to the overhead involved in the inclusion of both \fcro{a} CP and CS.


